Sample Preparation Meets Farey Sequence: A New Design Technique for Free-Flowing Microfluidic Networks

Design of microfluidic biochips has led to newer challenges to the EDA community due to the availability of various flow-based architectures and the need for catering to diverse applications such as sample preparation, personalized medicine, point-of-care diagnostics, and drug design. The ongoing Covid-19 pandemic has increased the demand for low-cost diagnostic lab-on-chips manifold. Sample preparation (dilution or mixing of biochemical fluids) is an indispensable step of any biochemical experiment including sensitive detection and successful assay execution downstream. Although for valve-based microfluidic biochips various design automation tools are currently available, they are expensive, and prone to various manufacturing and operational defects. Additionally, many problems are left open in the domain of free-flowing biochips, where only a single layer of flow-channels is used for fluid-flow devoid of any kind of control layer/valves. In this work, we present a methodology for designing a free-flowing biochip that is capable of performing fluid dilution according to users requirement. The proposed algorithm for sample preparation utilizes the Farey-sequence arithmetic of fractions that are used to represent the concentration factor of the target fluid. We also present the detailed layout design of a free-flowing microfluidic architecture that emulates the dilution algorithm. The network is simulated using COMSOL multi-physics software accounting for relevant hydrodynamic parameters. Experiments on various test-cases support the efficacy of the proposed design in terms of accuracy, convergence time, reactant cost, and simplicity of the fluidic network compared to prior art.

==> Algorithms/Algo1.tex <==
\begin{algorithm}[t]%!t]%h]
	%\tiny
	\small
	\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
	\let\oldnl\nl% Store \nl in \oldnl
	\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
	\KwIn{Accuracy \textit{n} (positive integer)}
	%{Desired target {\em CF} $C_t$, accuracy $n$ and array of micro-electrode {\em N$\times$N} equivalent
	%to an electrode size of conventional {\em DMFB}}
	\KwOut{\emph{FSD} sequence of order $2^{n}$.
	}
	Generate bit-scanning (\emph{BS}) sequence of order \emph{n}; i.e., $BS_{n}$ = \{$\frac{0}{2^{n}}$, $\frac{1}{2^{n}}$, $\frac{2}{2^{n}}$, .... , $\frac{2^{n}-1}{2^{n}}$, $\frac{2^{n}}{2^{n}}$\}\;
	
	Generate Farey (\emph{F}) sequence of order \emph{m} (where \emph{m} = $2^{n+1}-3$); i.e., $F_{m}$ = \{$\frac{0}{m}$, $\frac{1}{m-1}$, $\frac{1}{m-2}$, .... , $\frac{m-1}{m}$, $\frac{m}{m}$\}\;
	
	Generate reduced Farey (\emph{RF}) sequence of order ${2^{n}}$ such as\;
	%Generate proper subset from Farey sequence of order m ($Fr_m$) and named it as reduced Farey (RFr) sequence of order ${2^{n}}$ such that it includes first and last elements of Farey sequence of order m (i.e. $Fr_{m}$) and all elements of $Fr_{m}$ where numerator is within close interval of [0 , ($2^{n}-1$)] with difference between denominator and numerator is less than $2^{n}$ ; i.e. ;\;
	\nonl \hspace{0.5mm} $RF_{2^{n}}$ $\subset$ $F_m$  and \;
	\nonl \hspace{0.5mm} $RF_{2^{n}}$ = \{x $\mid$ x $\in$ \{$\frac{0}{2^{n}}$, $\frac{\phi}{\psi}$,  $\frac{2^{n}}{2^{n}}$\} \}\;
	\nonl \hspace{0.5mm} where  $\frac{\phi}{\psi}$ $\in$ $F_m$, and 0 $<$ $\phi$ $<$  $2^{n}$ and $\psi$ - $\phi$ $<$ $2^{n}$\;
	%\nonl \hspace{0.5mm} $RF_{2^{n}}$ = \{x $\mid$ x $\in$ \{$\frac{0}{2^{n}}$, $\frac{\phi}{\psi}$,  $\frac{2^{n}}{2^{n}}$\} \}\;
	%\nonl \hspace{0.5mm} where $\frac{\phi}{\psi}$ $\forall$  (0 $<$ $\phi$ $<$  $2^{n}$) $\wedge$ (($\psi$ - $\phi$) $<$ $2^{n}$) and $\phi$ \& $\psi$ both are positive integer.\;
	
	Generate \emph{FSD} sequence of order  ${2^{n}}$ such that \;
	%Generate proper subset from reduced Farey sequence of order $2^{n}$ ($RFr_{2^{n}}$) and named it as Farey Sequence based  Dilution preparation (FSD) sequence of order  ${2^{n}}$ such that \;
	\nonl \hspace{0.5mm} $FSD_{2^{n}}$ $\subset$ $RF_{2^{n}}$  and \;
	\nonl \hspace{0.5mm} $FSD_{2^{n}}$ = \{ x $\mid$ x $\in$ $\frac{0}{2^{n}}$, $\frac{\phi}{\psi}$, $\frac{2^{n}}{2^{n}}$ \}\;
	\nonl \hspace{0.5mm} where $\frac{\phi}{\psi}$ $\in$ \{$BS_n$\} $\vee$ \;
	\nonl \hspace{5mm}\{$\frac{t}{2^{n}}$ $<$ $\frac{\phi}{\psi}$ $<$ $\frac{2t+1}{2^{n+1}}$ $\mid$ $\phi$ is minimum among all numerator between open interval of ($\frac{t}{2^{n}}$,$\frac{2t+1}{2^{n+1}}$) \}  $\vee$ \;
	\nonl \hspace{5mm}\{$\frac{2t+1}{2^{n+1}}$ $<$ $\frac{\phi}{\psi}$ $<$ $\frac{t+1}{2^{n}}$ $\mid$ $\phi$ is minimum among all numerator between open interval of ($\frac{2t+1}{2^{n+1}}$,$\frac{t+1}{2^{n}}$) \} 
	
	\Return{ $FSD_{2^{n}}$}\;
	
	\caption{Generation of FSD Sequence}
	\label{algo:FSDGen}
\end{algorithm}

Step-wise explanation:

Step1: \textcolor{blue}{Generate bit-scanning (BS) sequence of order n ; i.e.; $BS_{n}$ = \{$\frac{0}{2^{n}}$, $\frac{1}{2^{n}}$, $\frac{2}{2^{n}}$, .... , $\frac{2^{n}-1}{2^{n}}$, $\frac{2^{n}}{2^{n}}$\};} [Need no explanation]

[Example: \emph{BS}$_3$ = \{$\frac{0}{2^{3}}$, $\frac{1}{2^{3}}$, $\frac{2}{2^{3}}$, .... , $\frac{2^{3}-1}{2^{3}}$, $\frac{2^{3}}{2^{3}}$\}]

\vspace{10pt}

Step 2: \textcolor{blue}{Generate Farey (\emph{F}) sequence of order m (where m = $2^{n+1}-3$) ; i.e.; $F_{m}$ = \{$\frac{0}{m}$, $\frac{1}{m-1}$, $\frac{1}{m-2}$, .... , $\frac{m-1}{m}$, $\frac{m}{m}$\};} [Need no explanation]

[Example: \emph{F}$_{13}$ = \{$\frac{0}{125}$, $\frac{1}{13}$, $\frac{1}{12}$, $\frac{1}{11}$, $\frac{1}{122}$,...,$\frac{10}{11}$, $\frac{11}{12}$, $\frac{12}{13}$, $\frac{13}{13}$\}]
\vspace{10pt}

Step 3:\textcolor{blue}{ Generate reduced Farey (\emph{RF}) sequence of order ${2^{n}}$ such as;} [Using this step we are going to generate a new sequence/set \emph{RF}$_{8}$ which has the following criteria ]

\textcolor{blue}{$RF_{2^{n}}$ $\subset$ $F_m$  and ;} [It is obvious, because \emph{RF}$_{2^n}$ is derived from \emph{F}$_m$; e.g., \emph{RF}$_{8}$ $\subset$ $F_{13}$ ]

\textcolor{blue}{\emph{RF}$_{2^{n}}$ = \{x $\mid$ x $\in$ \{$\frac{0}{2^{n}}$, $\frac{\phi}{\psi}$,  $\frac{2^{n}}{2^{n}}$\} \} }

\textcolor{blue}{where  $\frac{\phi}{\psi}$ $\in$ $F_m$,} [Each element $\frac{\phi}{\psi}$ of \emph{RF}$_{2^{n}}$ belongs to $F_m$]

\textcolor{blue}{and 0 $<$ $\phi$ $<$  $2^{n}$} [Numerator of each $\frac{\phi}{\psi}$ (i.e., $\phi$) must be within open interval of 0 \& $2^n$, i.e., (0, $2^n$). Reason: Our proposed diluter network, in support of accuracy $n$, has inlet arm widths (both for sample \& buffer inlets) of set like \{1, $2^1$, $2^2$, ..., $2^{n-1}$\} units. Hence, activation of all sample inlets at a time can inject ($2^n$ -1) units sample-fluid. Note, ($2^n$ -1) is simply sum of \{1, $2^1$, $2^2$, ..., $2^{n-1}$\}; i.e., (1 + $2^1$ + $2^2$ + ... + $2^{n-1}$) = $\sum_{i = 0}^{n-1}2^i$ = $2^n$ -1. Thus numerator value $\phi$, which represents the required units of sample fluid, can not exist ($2^n$ -1). And lower bound of $\phi$ must be greater than $0$, since some units of sample fluid should present in the dilution.]

\textcolor{blue}{and $\psi$ - $\phi$ $<$ $2^{n}$\;} [Difference between denominator $ \psi$ \& numerator $\phi$ represents the units of buffer fluid used in the dilution to achieve \emph{tCF} = $\frac{\phi}{\psi}$. As described in the above, upper bound of used units of buffer fluid is similar like sample fluid concept. Hence, activation of all buffer inlets at a time can inject ($2^n$ -1) units buffer fluid. Note, ($2^n$ -1) is simply sum of \{1, $2^1$, $2^2$, ..., $2^{n-1}$\}; i.e., (1 + $2^1$ + $2^2$ + ... + $2^{n-1}$) = $\sum_{i = 0}^{n-1}2^i$ = $2^n$ -1. Thus, again ($\psi$ - $\phi$), which represents the required units of buffer fluid, can not exist ($2^n$ -1). \textcolor{red}{Note, order of \emph{RF} is set to $2^n$ because of these two upper bound values.}]

[Example: \emph{RF}$_8$ =\{0, 1/8, 1/7, 1/6, 1/5, 2/9, 1/4, ..., 7/9, 4/5, 5/6, 6/7, 7/8, 1\}]
\vspace{10pt}

Step 4: \textcolor{blue}{ Generate \emph{FSD} sequence of order  ${2^{n}}$ such that }

\textcolor{blue}{\emph{FSD}$_{2^{n}}$ $\subset$ \emph{RF}$_{2^{n}}$} [Again, it is obvious as \emph{FSD}$_{2^{n}}$ is derives from \emph{RF}$_{2^{n}}$.]

\textcolor{blue}{and \emph{FSD}$_{2^{n}}$ = \{ x $\mid$ x $\in$ $\frac{0}{2^{n}}$, $\frac{\phi}{\psi}$, $\frac{2^{n}}{2^{n}}$ \}} 

\textcolor{blue}{where $\frac{\phi}{\psi}$ $\in$ \{$BS_n$\}} [$\frac{\phi}{\psi}$ is an element of the set \{$BS_n$\}. Because, our target is to generate a sequence in such a way that contains all elements of $BS_n$ as well as two more elements in each two consecutive elements in the $BS_n$ sequence to reduce error value ($< 0.5$) and simultaneously delete the constraint (i.e., denominator should be power of 2) over denominator. Hence, \emph{FSD}$_{2^{n}}$ should be a proper super-set of $BS_n$ (i.e., \emph{FSD}$_{2^{n}}$ $\supset$ $BS_n$). It is possible. Because, Farey sequence of order $m$, \emph{F}$_{m(=2^{n+1}-3)}$, contains irreducible rational numbers $\frac{a}{b}$ with $0 \le a \le b \le m$ and (a,b)=1 arranged in increasing order. \emph{RF}$_{2^n}$ is the proper subset of \emph{F}$_m$ having all numerator values within open interval (0, $2^n$) and difference between denominator \& numerator is also within open interval (0, $2^n$). Notice that, $BS_n$ also contains such elements which satisfy these two conditions -- all numerator values within open interval (0, $2^n$) and difference between denominator \& numerator is also within open interval (0, $2^n$) along with all denominators are $2^n$. Hence, \emph{RF}$_{2^n}$ $\supset$ $BS_n$ and \emph{FSD}$_{2^{n}}$ $\subset$ \emph{RF}$_{2^{n}}$. Through next two constraints, we'll see how $|$\emph{FSD}$_{2^{n}}$$|$ is become greater than $|$$BS_n$$|$.]

\textcolor{blue}{$\vee$} [OR]

\textcolor{blue}{\{$\frac{t}{2^{n}}$ $<$ $\frac{\phi}{\psi}$ $<$ $\frac{2t+1}{2^{n+1}}$ $\mid$ $\phi$ is minimum among all numerators between open interval of ($\frac{t}{2^{n}}$,$\frac{2t+1}{2^{n+1}}$) \}} [Let us consider two consecutive elements from $BS_n$ sequence are $\frac{t}{2^n}$ \& $\frac{t+1}{2^n}$. Now, middle element of these two elements is $\frac{2t+1}{2^{n+1}}$ (= \{$\frac{t}{2^n}$ + $\frac{t+1}{2^n}$\}/2). Next, we choose $\frac{\phi}{\psi}$ in such a way that numerator $\phi$ is minimum among all numerators between open interval of the lower half; i.e., ($\frac{t}{2^{n}}$,$\frac{2t+1}{2^{n+1}}$) which implies minimum use of sample. Hence cost effective.]

[Example: For t=1, n=3 we have 1/6 within (1/8, 3/16)]

\textcolor{blue}{$\vee$} [OR]

\textcolor{blue}{\{$\frac{2t+1}{2^{n+1}}$ $<$ $\frac{\phi}{\psi}$ $<$ $\frac{t+1}{2^{n}}$ $\mid$ $\phi$ is minimum among all numerator between open interval of ($\frac{2t+1}{2^{n+1}}$,$\frac{t+1}{2^{n}}$) \}} [Same search as mention just above but within open interval of the upper half; i.e., ($\frac{2t+1}{2^{n+1}}$,$\frac{t+1}{2^{n}}$).]

[Example: For t=1, n=3 we have 1/5 within (3/16, 1/4)]

[\textcolor{red}{Note, in this way we can claim \emph{FSD}$_{2^{n}}$ $\supset$ $BS_n$\\
and $|$\emph{FSD}$_{2^{n}}$$|$ $>$ $|$$BS_n$$|$}]

[Example: \emph{FSD}$_{8}$ = \{0, 1/8, 1/6, 1/5, 1/4, ..., 5/6, 7/8, 1\}]
\begin{figure}[h]
	\centering
	\includegraphics[width=9.1cm,keepaspectratio]{BDP4mFarey.pdf}
	\caption{Derivation of $FSD_{8}$ sequence from $F_{13}$}%\todo[inline]{change BS3 $-->$ GS3}}
	\label{fig:FSD4mFarey}
\end{figure}



==> Algorithms/Algo2.tex <==
\begin{algorithm}[!h]%!t]%h]
	%\small
	\scriptsize
	\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
	\let\oldnl\nl% Store \nl in \oldnl
	\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
	\KwIn{Accuracy $n$, an ordered sequence \textit{$ \xi$} with proper fractions in $[0,1]$ and target \textit{CF} (\emph{tCF})}
	%{Desired target {\em CF} $C_t$, accuracy $n$ and array of micro-electrode {\em N$\times$N} equivalent
	%to an electrode size of conventional {\em DMFB}}
	\KwOut{An element from the ordered sequence $\xi$ with error $\epsilon$
	}
	
	Express \emph{tCF} as $\frac{\phi}{\psi}$ such that 0 $\leq$ $\phi$ $\leq$ $\psi$\;
	\{$\frac{\phi_1}{\psi_1}$,  $\frac{\phi_2}{\psi_2}$\, $PoS_1$, $PoS_2$\} = \Call{SearchRange}{$\frac{\phi}{\psi}$, $\xi$}\;
	\If{$PoS_1$ = $PoS_2$}{$\epsilon$ = $\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_1}{\psi_1}$, $\epsilon$}}
	\If{$PoS_1$ - $PoS_2$ = 1}{\eIf{($\frac{\phi}{\psi}$ - $\frac{\phi_1}{\psi_1}$) $<$ ($\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$)} {$\epsilon$ = $\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$; %\;
			\Return{$\frac{\phi_1}{\psi_1}$, $\epsilon$}}{$\epsilon$ = $\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$; %\;
			\Return{$\frac{\phi_2}{\psi_2}$, $\epsilon$}}}
	%\Return{ \textit{$SEQ_{S}$}, $\overline{SEQ_S}$, \textit{$SEQ_{B}$}}, and $\overline{SEQ_B}$\;
	$y_1$ = ($\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$) \&  $y_2$ = ($\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$)\;
	%\nonl $y_2$ = $\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$\;
	$x\mid_{y = 0}$ = $\frac{PoS_1\cdot y_2 - PoS_2\cdot y_1}{y_2 - y_1}$\;
	$\frac{\phi_3}{\psi_3} = \lfloor x \rfloor^{th}$ element of $\xi$\;
	\eIf{$\frac{\phi_3}{\psi_3}$ $\leqslant$ $\frac{\phi}{\psi}$}{$\frac{\phi_4}{\psi_4} = \lfloor x+1 \rfloor^{th}$ element of $\xi$}{$\frac{\phi_4}{\psi_4} = \lfloor x-1 \rfloor^{th}$ element of $\xi$}%\;
	\eIf{$\frac{\phi_3}{\psi_3}$ $\leqslant$ $\frac{\phi}{\psi}$ $\leqslant$ $\frac{\phi_4}{\psi_4}$ }{\eIf{($\frac{\phi}{\psi}$ - $\frac{\phi_3}{\psi_3}$) $<$ ($\frac{\phi_4}{\psi_4}$ - $\frac{\phi}{\psi}$)}{$\epsilon$ = $\frac{\phi_3}{\psi_3}$ - $\frac{\phi}{\psi}$; %\;
			\Return{$\frac{\phi_3}{\psi_3}$, $\epsilon$}}{$\epsilon$ = $\frac{\phi_4}{\psi_4}$ - $\frac{\phi}{\psi}$; %\;
			\Return{$\frac{\phi_4}{\psi_4}$, $\epsilon$}}}{\eIf{$\frac{\phi}{\psi}$ $<$ $\frac{\phi_3}{\psi_3}$}{$\frac{\phi_2}{\psi_2}$ = $\frac{\phi_3}{\psi_3}$;  %\; 
			\textbf{goto} Step 10}{$\frac{\phi_1}{\psi_1}$ = $\frac{\phi_4}{\psi_4}$; %\;
			\textbf{goto} Step 10}} 
	\begin{algorithmic}%[l]
		%\small
		\scriptsize
		\DontPrintSemicolon
		\Procedure{SearchRange}{$\frac{\phi}{\psi}$, $\xi$}:\;
		$G_1$ = GCD($\lfloor(\phi n)/\psi\rfloor,n$) and %\;
		$G_2$ = GCD($\lceil(\phi n)/\psi\rceil,n$)\;
		$\phi_1$ = $\lfloor(\phi n)/\psi\rfloor/G_1$ and $\phi_2$ = $\lceil(\phi n)/\psi\rceil/G_2$\;%\;
		$\psi_1$ = $n/G_1$ and $\psi_2$ = $n/G_2$\;
		$PoS_1$ = position of $\frac{\phi_1}{\psi_1}$ in $\xi$\;
		$PoS_2$ = position of $\frac{\phi_2}{\psi_2}$ in $\xi$\;
		%\Comment{\parbox[t]{0.5\linewidth}{open the green valve of the sample inlet arm towards the mixing chamber at time $ \Gamma $;}} \;
		
		%\Comment{\parbox[t]{.5\linewidth}{ open the red valve of the sample inlet arm towards the reuse chamber at time $ \Gamma $;}}\;
		\Return $\frac{\phi_1}{\psi_1}$, $\frac{\phi_2}{\psi_2}$, $PoS_1$, $PoS_2$\;
		\EndProcedure
	\end{algorithmic}
	%	\caption{\textcolor{red}{Mapping to minimum error \textit{CF} }}
	\caption{Mapping to minimum error \textit{CF} }
	\label{algo:Mapping}
\end{algorithm}

Step-wise explanation:\\

\textcolor{blue}{INPUT: Accuracy $n$, an ordered sequence \textit{$ \xi$} with proper fractions in $[0,1]$ and target \textit{CF} (\emph{tCF})}

[Ordered sequence \textit{$ \xi$} means \emph{FSD} sequence, the output of Algo 1]\\

Step 1: \textcolor{blue}{Express \emph{tCF} as $\frac{\phi}{\psi}$ such that 0 $\leq$ $\phi$ $\leq$ $\psi$}

[Convert the value of \emph{tCF} (may be in \% form) into fractional form]\\

Step 2: \textcolor{blue}{\{$\frac{\phi_1}{\psi_1}$,  $\frac{\phi_2}{\psi_2}$\, $PoS_1$, $PoS_2$\} = \Call{SearchRange}{$\frac{\phi}{\psi}$, $\xi$}}

[shorten the search range to map \emph{tCF} to its nearest value (which in tern provides smaller error). Here $\frac{\phi_1}{\psi_1}$ is the lower bound of the search range which is at $({PoS_1})^{th}$ position in the list. Similarly, $\frac{\phi_2}{\psi_2}$ is the upper bound of the search range which is at $({PoS_2})^{th}$ position in the list]\\

Step 3 \& 4: \textcolor{blue}{\If{$PoS_1$ = $PoS_2$}{$\epsilon$ = $\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_1}{\psi_1}$, $\epsilon$}}}

[This means, exact mapping is found for the \emph{tCF}]\\

Step 5: \textcolor{blue}{if ($PoS_1$ - $PoS_2$ = 1)}

[If lower \& upper bounds are at 2 consecutive positions]

Step 6 to 9: \textcolor{blue}{\eIf{($\frac{\phi}{\psi}$ - $\frac{\phi_1}{\psi_1}$) $<$ ($\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$)} {$\epsilon$ = $\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_1}{\psi_1}$, $\epsilon$}}{$\epsilon$ = $\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_2}{\psi_2}$, $\epsilon$}}}

[Then simply choose that bound value which provide small error; i.e., nearest value]\\ 

Step 10: \textcolor{blue}{$y_1$ = ($\frac{\phi_1}{\psi_1}$ - $\frac{\phi}{\psi}$) \&  $y_2$ = ($\frac{\phi_2}{\psi_2}$ - $\frac{\phi}{\psi}$)}

[Set $y_1$ as difference between lower bound \& \emph{tCF}, and $y_2$ as difference between upper bound \& \emph{tCF}]\\

Step 11: \textcolor{blue}{$x\mid_{y = 0}$ = $\frac{PoS_1\cdot y_2 - PoS_2\cdot y_1}{y_2 - y_1}$}

[Find the ``zero-crossing" and set that position at $x$]\\

Step 12: \textcolor{blue}{$\frac{\phi_3}{\psi_3} = \lfloor x \rfloor^{th}$ element of $\xi$}

[Set $\lfloor x \rfloor^{th}$ element of the sequence $\xi$ as one of the new bound of the \emph{tCF}]\\

Step 13 \& 16: \textcolor{blue}{\eIf{$\frac{\phi_3}{\psi_3}$ $\leqslant$ $\frac{\phi}{\psi}$}{$\frac{\phi_4}{\psi_4} = \lfloor x+1 \rfloor^{th}$ element of $\xi$}{$\frac{\phi_4}{\psi_4} = \lfloor x-1 \rfloor^{th}$ element of $\xi$}}

[If the new bound $\frac{\phi_3}{\psi_3}$ can be taken as lower bound of the \emph{tCF}, then $\lfloor x+1 \rfloor^{th}$ element of the sequence $\xi$ will be set as upper bound $\frac{\phi_4}{\psi_4}$ of the \emph{tCF}. Otherwise, $\frac{\phi_3}{\psi_3}$ become upper bound and lower bound $\frac{\phi_4}{\psi_4}$ will be the $ \lfloor x-1 \rfloor^{th}$ element of the sequence $\xi$]\\

Step 17: \textcolor{blue}{if ($\frac{\phi_3}{\psi_3}$ $\leqslant$ $\frac{\phi}{\psi}$ $\leqslant$ $\frac{\phi_4}{\psi_4}$ ) then}

[If $\frac{\phi}{\psi}$ lies within closed interval of [$\frac{\phi_3}{\psi_3}$, $\frac{\phi_4}{\psi_4}$] then reach the nearest value]\\

Step 18 to 21: \textcolor{blue}{\eIf{($\frac{\phi}{\psi}$ - $\frac{\phi_3}{\psi_3}$) $<$ ($\frac{\phi_4}{\psi_4}$ - $\frac{\phi}{\psi}$)}{$\epsilon$ = $\frac{\phi_3}{\psi_3}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_3}{\psi_3}$, $\epsilon$}}{$\epsilon$ = $\frac{\phi_4}{\psi_4}$ - $\frac{\phi}{\psi}$; %\;
		\Return{$\frac{\phi_4}{\psi_4}$, $\epsilon$}}}

[Which one provide smaller error for $\frac{\phi}{\psi}$, will be the nearest value]\\

Step 22: \textcolor{blue}{else}

[Otherwise need to modify search range]\\

Step 23 to 26: \textcolor{blue}{\If{$\frac{\phi}{\psi}$ $<$ $\frac{\phi_3}{\psi_3}$}{$\frac{\phi_2}{\psi_2}$ = $\frac{\phi_3}{\psi_3}$;  %\; 
		\textbf{goto} Step 10}{$\frac{\phi_1}{\psi_1}$ = $\frac{\phi_4}{\psi_4}$; %\;
		\textbf{goto} Step 10}}

[If $\frac{\phi}{\psi}$ is still less than $\frac{\phi_3}{\psi_3}$, then set the new search range as ($\frac{\phi_1}{\psi_1}$, $\frac{\phi_3}{\psi_3}$) and go to step 10. Otherwise, set the new search range as ($\frac{\phi_4}{\psi_4}$, $\frac{\phi_2}{\psi_2}$) and go to step 10.]\\

[Example: Applying this algorithm for $n$ = $6$, $\xi$ = \emph{FSD}$_{64}$, and \emph{tCF} = $69.3\%$ (=$\frac{44.375}{64}$), we received $\frac{9}{13}$ as the nearest \emph{CF} value with minimum error (here, $\epsilon$ = $\frac{0.067}{64}$)]\\

Let us consider an example to explain the working principle of Algorithm \ref{algo:Mapping}. We start with accuracy $n$ = $6$, an ordered sequence $\xi$ (here it is output of Algorithm \ref{algo:FSDGen} for $n$ = $6$; i.e., \emph{FSD}$_{64}$), and a target-\emph{CF} \emph{tCF} = $69.3\%$. As per step 1, we set \emph{tCF} = $69.3\%$ = $\frac{44.375}{64}$. Now applying the procedure to generate a compact search range for \emph{tCF} = $\frac{44.375}{64}$ in the \emph{FSD}$_{64}$ sequence, we receive a search range from $127^{th}$ (\emph{PoS$_1$}) element $\frac{2}{3}$ ($\frac{\phi_1}{\psi_1}$) to $189^{th}$ (\emph{PoS$_2$}) element $\frac{1}{1}$ ($\frac{\phi_2}{\psi_2}$). In this case difference between \emph{PoS$_1$} and \emph{PoS$_2$} is greater than 1, so we directly go to step 10. Here, we set $y_1$ as difference between lower bound \& \emph{tCF} (i.e., $y_1$ = $\frac{2}{3}$ - $\frac{44.375}{64}$ = $-0.026666667$), and $y_2$ as difference between upper bound \emph{tCF} (i.e., $y_2$ = $\frac{1}{1}$ - $\frac{44.375}{64}$ = $0.306666667$). At next, we find the “zero-crossing” \cite{FareyPB} and set that position at $x$, where $x$ is now equal to $131.9648438$. We need to make search range more close to our target. So, set $\lfloor x \rfloor^{th}$ element of the sequence $\xi$ or \emph{FSD}$_{64}$ as one of the new bound of our target; i.e., $\frac{\phi_3}{\psi_3}$ = $\frac{11}{16}$. Let see, whether it is new lower bound or upper bound through steps $13$ to $16$. Since, $\frac{\phi_3}{\psi_3}$ (= $\frac{11}{16}$) is less than $\frac{\phi}{\psi}$ (= $\frac{44.375}{64}$), $\frac{11}{16}$ is new lower bound, and new upper bound $\frac{\phi_4}{\psi_4}$  is equal to $\lfloor x + 1 \rfloor^{th}$ element of the sequence $\xi$ or \emph{FSD}$_{64}$; i.e., $\frac{\phi_4}{\psi_4}$ = $\frac{9}{13}$. We can see that $\frac{44.375}{64}$ is lies between closed interval of [$\frac{11}{16}$, $\frac{9}{13}$]. Since $\frac{\phi}{\psi}$ - $\frac{\phi_3}{\psi_3}$ (i.e., $\frac{44.375}{64}$ - $\frac{11}{16}$ = $0.005859375$) is greater than $\frac{\phi_4}{\psi_4}$ - $\frac{\phi}{\psi}$ (i.e., $\frac{9}{13}$ - $\frac{44.375}{64}$ = $-0.001051683$), we achieve the nearest value which is $\frac{\phi_4}{\psi_4}$ = $\frac{9}{13}$ with minimum error $\epsilon$ = $-0.001051683$ = $-\frac{0.07}{64}$. Here, we can highlight that error $\epsilon$ = $\frac{44}{64}$ - $\frac{44.375}{64}$ = $-\frac{0.375}{64}$ while using $\xi$ = $BS_6$ sequence. Since, $|-\frac{0.07}{64}|$ is less than $|-\frac{0.375}{64}|$, we can conclude that approximating \emph{tCF} using proposed \emph{FSD}$_{2^n}$ sequence is more accurate than that of \emph{BS}$_{n}$ sequence.






==> Algorithms/Algo3.tex <==
\begin{algorithm}[!h]%h]
	%\small
	\scriptsize
	\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
	\KwIn{Sample concentration-factor $\textit{CF}_S$ , buffer $\textit{CF}_B$ and target \textit{CF} (\emph{tCF})}
	%{Desired target {\em CF} $C_t$, accuracy $n$ and array of micro-electrode {\em N$\times$N} equivalent
	%to an electrode size of conventional {\em DMFB}}
	\KwOut{Fluid injection sequences by controlling ON/OFF sequences of valves:\; for sample/reactant these are represented by \textit{$SEQ_{S}$}, $\overline{{SEQ_{S}}}$ (controlling valves to make the fluid flow towards mixing and reuse chambers, respectively) and \textit{$SEQ_{B}$}, $\overline{{SEQ_{B}}}$ are stand for same purpose, but for buffer
	}
	Express \emph{tCF} as $\frac{\phi}{\psi}$\;
%	Let us assume that start time of first fluid injection is $ \Gamma $\;
	Compute required unit of Sample : $ \phi $ unit of Sample \;
	Compute required unit of Buffer : $ \varphi(=\psi-\phi) $ unit of buffer\;
	Convert $ \phi $ and $ \varphi $ into 6 bits binary values i.e. $ \phi_{bin} $ and $ \varphi_{bin} $ respectively\;
	\While{scan $ \phi_{bin} $ and $\varphi_{bin}$ from right to left}{
		%\For{right most scan bit or say least significant bit (\textit{LSB}) of both $ \phi_{bin} $ and $\varphi_{bin}$}{
			$SEQ_S$ = \Return \Call{GenSequence}{scan bit of $\phi_{bin}$,  $SEQ_{S}$}\;
			$SEQ_B$ = \Return \Call{GenSequence}{scan bit of $\varphi_{bin}$, $SEQ_{B}$}\;
		%}
		%Set $ \Gamma = \Gamma + 5$  \;
		%$SEQ_S$ = \Return \Call{GenSequence}{scan bit of $\phi_{bin}$, $\Gamma$, $SEQ_{S}$}\;
		%Set $ \Gamma = \Gamma + 5$  \;
		%$SEQ_B$ = \Return \Call{GenSequence}{scan bit of $\varphi_{bin}$, $\Gamma$, $SEQ_{B}$}\;  
	}
	Append complement values of $SEQ_S$ to $\overline{SEQ_S}$\;
	Append complement values of $SEQ_B$ to $\overline{SEQ_B}$\;
	\Return{ \textit{$SEQ_{S}$}, $\overline{SEQ_S}$, \textit{$SEQ_{B}$}}, and $\overline{SEQ_B}$\;
	
	\begin{algorithmic}%[l]
		\small
		\DontPrintSemicolon
		\Procedure{GenSequence}{$\theta$, $SEQ$}:\;
		\eIf{$ \theta $ is 1}{
			Append ``ON" to $SEQ$
			\Comment{\parbox[t]{0.3\linewidth}{open the valve of the inlet arm towards the mixing chamber;}} \;
		}{
			Append ``OFF" to $SEQ$
			\Comment{\parbox[t]{.3\linewidth}{ close the valve of the inlet arm towards the mixing chamber;}}\;
		}
		\Return $SEQ$\;
		\EndProcedure
	\end{algorithmic}
	%\caption{\textcolor{red}{Off-line Valve Set-Up}}
	\caption{Off-line Valve Set-Up}
	\label{algo:SEQ_gen}
\end{algorithm}

Step-wise explanation:\\

\textcolor{blue}{INPUT: Target \textit{CF} (\emph{tCF})}

[Example: \emph{tCF} = 69.23\%]\\

Step 1: \textcolor{blue}{Express \emph{tCF} as $\frac{\phi}{\psi}$}

[Example: \emph{tCF} = 69.23\% = $\frac{9}{13}$ (output of Algo2)]\\


%Step 2: \textcolor{blue}{Let us assume that start time of first fluid injection is $ \Gamma $}
%
%[Example: Let $\Gamma$ = $5 sec$]\\

Step 2: \textcolor{blue}{Compute required unit of Sample : $ \phi $ unit of Sample}

[Example: Here $\phi$ = $9$]\\

Step 3: \textcolor{blue}{Compute required unit of Buffer : $ \varphi(=\psi-\phi) $ unit of buffer}

[Example: $ \varphi$ = $\psi-\phi $ = $13 - 9$ = $4$; i.e., mixing of 9 units of sample/reactant with 4 (= 13-9) units of buffer can prepare 69.23\% diluted sample. ]\\

Step 4: \textcolor{blue}{Convert $ \phi $ and $ \varphi $ into 6 bits binary values i.e. $ \phi_{bin} $ and $ \varphi_{bin} $ respectively}

[Example: $ \phi $ = $(9)_{10}$ $\Rightarrow$  $ \phi_{bin} $ =$(001001)_2$

$ \varphi $ = $(4)_{10}$ $\Rightarrow$ $ \varphi_{bin} $ = $(000100)_2$
 
Why 6? Because, accuracy $n$ = $6$ = $\#$ of sample inlets = $\#$ of buffer inlets]\\
 
Step 5: \textcolor{blue}{While (scan $ \phi_{bin} $ and $\varphi_{bin}$ from right to left)}

[Start to scan the binary values from right to left; i.e, from least significant bit (\textit{LSB}) to most significant bit (\textit{MSB}). Take one scan bit from sample/reactant, then one scan bit from buffer, again next higher one from sample, and then buffer, and so on upto completing the scan of all 12 bits.]
	
\textcolor{blue}{\{ }[Do the followings:]
		
%\textcolor{blue}{For (right most scan bit or say least significant bit (\textit{LSB}) of both $ \phi_{bin} $ and $\varphi_{bin}$)}

[Start with \emph{LSB} from both $ \phi_{bin} $ and $\varphi_{bin}$

Example: $ \phi_{bin} $ =$(00100\textcolor{red}{1})_2$ and $ \varphi_{bin} $ = $(00010\textcolor{red}{0})_2$]

%\textcolor{blue}{\{}[Do the followings:]
	
Step 6: \textcolor{blue}{$SEQ_S$ = \Return \Call{GenSequence}{scan bit of $\phi_{bin}$, $SEQ_{S}$}}

[\textit{$SEQ_{S}$} = controlling valve sequence to make the sample fluid flow towards mixing chamber

If scan bit is $1$ then append ``ON" to \textit{$SEQ_{S}$}

If scan bit is $0$ then append ``OFF" to \textit{$SEQ_{S}$}]

Step 7: \textcolor{blue}{$SEQ_B$ = \Return \Call{GenSequence}{scan bit of $\varphi_{bin}$, $SEQ_{B}$}}

[\textit{$SEQ_{B}$} =  controlling valve sequence to make the buffer fluid flow towards mixing chamber

If scan bit is $1$ then append ``ON" to \textit{$SEQ_{B}$}

If scan bit is $0$ then append ``OFF" to \textit{$SEQ_{B}$}]

\textcolor{blue}{\}}

Step 8: \textcolor{blue}{Append complement values of $SEQ_S$ to $\overline{SEQ_S}$}

[$\overline{SEQ_S}$ = controlling valve sequence to make the sample fluid flow towards reuse chamber.

According to our model, fluids can be injected towards either mixing channel or reuse channel. Thus, valve controlling sequence for a particular inlet must has two complement values (states of valves) in the direction of mixer and reuse chamber]

Step 9: \textcolor{blue}{Append complement values of $SEQ_B$ to $\overline{SEQ_B}$}

[$\overline{SEQ_B}$ = controlling valve sequence to make the sample fluid flow towards reuse chamber.]
%\textcolor{blue}{Set $ \Gamma = \Gamma + 5$}
%
%\textcolor{blue}{$SEQ_S$ = \Return \Call{GenSequence}{scan bit of $\phi_{bin}$, $\Gamma$, $SEQ_{S}$}}
%
%\textcolor{blue}{Set $ \Gamma = \Gamma + 5$ }
%
%\textcolor{blue}{$SEQ_B$ = \Return \Call{GenSequence}{scan bit of $\varphi_{bin}$, $\Gamma$, $SEQ_{B}$}}
%
%\textcolor{blue}{\}}

Step 10: \textcolor{blue}{\Return{ \textit{$SEQ_{S}$}, $\overline{SEQ_S}$, \textit{$SEQ_{B}$}, and $\overline{SEQ_B}$}}

[Example: For \emph{tCF} = 69.23\% = $\frac{9}{13}$, we have the following valve controlling sequences after the execution og this algorithm:

$SEQ_{S}$ = \{ON, OFF, OFF, ON, OFF, OFF \}

$\overline{SEQ_S}$ = \{OFF, ON, ON, OFF, ON, ON\}

\textit{$SEQ_{B}$} = \{OFF, OFF, ON, OFF, OFF, OFF\}

$\overline{SEQ_B}$ = \{ON, ON, OFF, ON, ON, ON\}]

\textcolor{red}{Note: I've modified the Algo 3. I've deleted the time constraint $\Gamma$. Because, if start time is $\Gamma$, then at $\Gamma$ first sample and buffer fluids are injected through extreme left inlets of our network. Then gradually fluid injection through each inlets (alternatively sample inlet then buffer inlet) will be started each after 5 sec towards right direction of the network. This timing is independent of target-\emph{CF}.}












==> Text/motivation_layout.tex <==
\noindent
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.3}
\begin{table*}[htbp]
	\caption[ \color{blue}Theoritical comparisions with prior-art]{ \color{blue}Scope of the proposed method compared to prior flow-based dilution algorithms}
	\label{table:obj_comapare}
	\scriptsize
	\begin{center}
		\begin{threeparttable} 
			\begin{tabular}{|p{2.1cm}|p{1.3cm}|p{2cm}|p{1.3cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1.4cm}|}
				\hline
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Method}} &
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Control-valve needed in the mixing channel?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Valve handling mechanism}}&	    
				\cellcolor{pink!16}
				\color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Error-tolerance limit}}& 
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Fluid-injection	sequence required?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Any fluid wasted?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Mix, split steps required?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \tiny How many different fluid-injection velocities used?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Physical design independent of target-\emph{CF}?}}\\ 
				%\midrule
				{ \raggedleft Wang {\em et al.}\cite{Philip2016}} & yes (?) & off-line & $>$1\% & no &no & yes, yes &  1 &  yes (fixed ratio) \\ \\
				
				{ \raggedleft Jeon {\em et al.}\cite{Xmas}} & no & valve-free & undefined & N/A &no  & yes, yes & 1 &  no \\ \\
				
				{ \raggedleft Lee {\em et al.} \cite{SerialDilution}} & no & free & undefined &N/A  &no & yes, yes & 1 &  no \\ \\ 
				
				{ \raggedleft Bhattacharjee {\em et al.}\cite{Rotary}} & yes & on-line & undifined  & yes &yes  & yes, yes & 1 &  yes \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{Banerjee2017}} & no & valve-free &  $\leq$ 0.5& yes  &no & yes, no & 2 &  yes\\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{BanerjeeVLSID2019}} & no & valve-free &  $\leq$ 0.5\% & yes  &no & yes, no & 2 &  yes \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{BanerjeeCBT}} & no & valve-free &  $\leq$ 0.5\% & yes  &no & yes, no & 1 &  yes \\ \\
				
				\cellcolor{cyan!16} \color{blue}{ \raggedleft [Proposed]} & \cellcolor{cyan!16} \color{blue}no & \cellcolor{cyan!16} \color{blue}valves needed only at the inputs; to be
				set in off-line mode & \cellcolor{cyan!16} \color{blue} $<$0.5\% &\cellcolor{cyan!16} \color{blue} no  \cellcolor{cyan!16} \color{blue}& \cellcolor{cyan!16} \color{blue}no, it is recycled & \cellcolor{cyan!16} \color{blue}yes, no &\cellcolor{cyan!16} \color{blue} 1 & \cellcolor{cyan!16} \color{blue}yes \\				
%				\bottomrule 
			\end{tabular} 
		\end{threeparttable}
	\end{center}
\end{table*}



==> tables/OnOff.tex <==
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[!h]%b]
%\caption{\color{red}{ON(1)-OFF(0) Sequences of Valves at Inlet Arms towards the Mixing Chambers for Different \emph{tCFs} (updated)}}
\caption{ON(1)-OFF(0) Sequences of Valves at Inlet Arms towards the Mixing Chambers for Different \emph{tCFs}}
\label{tb2:on_off_sequence}
\begin{center}
 \begin{tabular}{|| >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm}|| >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm} >{\small}p{0.5cm}|| >{\small}p{0.7cm}||}
 	
 \hline
 \multicolumn{6}{||c||}{\small{Sample}} & \multicolumn{6}{c||}{\small{Buffer}} & \multicolumn{1}{c||}{\small{tCF}}\\
 \hhline{------------~} 
    {1}  & {2}  & {4}  & {8}  & {16} & {32} & {1}  & {2}  & {4}  & {8}  & {16} & {32} & \multicolumn{1}{c||}{\small{in \%}}\\ 
 \hline 

1	&0	&0	&0	&0 &0	&1	&1	&1	&1	&1	&0 &3	\\ 
1	&0	&0	&0	&0	&0 &0	&1	&1	&1	&1	&0 &3.25	\\
1	&0	&0	&0	&0	&0 &1	&1	&1	&0	&0 &0	&12.5	\\
1	&0	&0	&1	&0	&0 &0	&0	&1	&0	&1	&0 &31	\\	
1	&0	&1	&0	&0	&0 &1	&1	&1	&0	&0	&0 &41.75	\\	
0	&1	&1	&0	&0	&0 &1	&0	&1	&0	&0	&0 &54.5	\\	
1	&0	&0	&1	&0	&0 &0	&0	&1	&0	&0 &0	&69.23	\\	
1	&1	&1	&0	&0	&0&1	&1	&0	&0	&0 &0	&70	\\	
1	&1	&1	&0	&0	&0 &1	&0	&0	&0	&0 &0	&87.5	\\
1	&1	&0	&0	&1	&0 &1	&0	&0	&0	&0 &0 &95	\\	\hline
\end{tabular}
\end{center}
\end{table}

==> tables/PriorWork.tex <==
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{table*}[!h]
	\caption[ \color{blue}Theoritical comparisions with prior-art]{ \color{blue}Scope of the proposed method compared to the state-of-the-art dilution algorithms}
	\label{table:obj_comapare}
	\scriptsize
	%\def\arraystretch{1}
	\begin{center}
		\begin{threeparttable} 
			%\resizebox{\columnwidth}{!}{%
			\begin{tabular}{|p{2.3cm}|p{1.2cm}|p{.85cm}|p{.8cm}|p{.9cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.4cm}|}%p{1cm}|p{1cm}|}%llllllll} 
				\toprule 
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Method}} &
				%			    \parbox[t]{1mm}{\rotatebox[origin=c]{90}{Valve use in mixing channel?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Valve use in mixing channel?}}&
				%			    {\raggedleft \rotatebox{90}{Valve use in mixing channel?}} &
				%                {\raggedleft \rotatebox{90}{Use of valve: on-line / off-line / free?}} & 
				%                \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Use of valve: on-line / off-line / free?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Valve handling mechanism}}&
				%                Valve handling mechanism
				%			    {\raggedleft  \rotatebox{90}{Error scale?}}&
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Error scale?}}&Error-tolerance limit
				%			    
				\cellcolor{pink!16}
				\color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Error-tolerance limit}}&
				%			    {\raggedleft  \rotatebox{90}{Is accuracy similar to accuracy of DMFB?}}&
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is accuracy similar to accuracy of DMFB?}}& 
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering achieves higher accuracy}}&
				%			    {\raggedleft  \rotatebox{90}{Is fluid-injection sequence specific?}} &
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is fluid-injection sequence specific?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is fluid-injection sequence target-specific?}}&
				%			    {\raggedleft  \rotatebox{90}{Are unused fluid recycled?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Are unused fluid recycled?}}&
				%			    {\raggedleft  \rotatebox{90}{Mix, Split?}} &
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Mix, Split?}}&
				%			    {\raggedleft  \rotatebox{90}{\# used fluid-injection velosity?}} &
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \# used fluid-injection velosity?}}&
				%			    {\raggedleft \rotatebox{90}{\emph{CF}-value at outlet (single / multiple / in a range)?}} &
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \emph{CF}-value at outlet (single / multiple / in a range)?}}&
				%			    # of CF-values produced?
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \# \emph{CF}-values produced}}&
				%				{\raggedleft \rotatebox{90}{Programmable?}}
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Programmable?}}\\ 
				\midrule
				{ \raggedleft Wang {\em et al.}\cite{Philip2016}} & yes (?) & off-line & $>$1\% &no& no &no & yes, yes &  1 & multiple (3) & yes (fixed ratio) \\ 
				
				{ \raggedleft Jeon {\em et al.}\cite{Xmas}} & no & valve-free & undefined &no& ? &no  & yes, yes & 1 & in a range & no \\ %\\
				
				{ \raggedleft Lee {\em et al.} \cite{SerialDilution}} & no & free & undefined &no& ?  &no & yes, yes & 1 & multiple (fixed) & no \\ %\\ 
				
				{ \raggedleft Bhattacharjee {\em et al.}\cite{Rotary}} & yes & on-line &   &no& ? &no  & yes, yes & 1 & yes & yes \\ %\\%(upto certain label) \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{Banerjee2017}} & no & valve-free &  $\leq$ 0.5&yes& yes  &no & yes, no & 2 & single & yes\\ %\\% &yes & yes  &no   & yes, no & 2 & single & yes \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{BanerjeeVLSID2019}} & no & valve-free &  $\leq$ 0.5\% &yes& yes  &no & yes, no & 2 & single & yes \\ %\\
				
				\cellcolor{cyan!16} \color{blue}{ \raggedleft [Proposed]} & \cellcolor{cyan!16} \color{blue}no & \cellcolor{cyan!16} \color{blue}off-line & \cellcolor{cyan!16} \color{blue} $<$0.5\% &\cellcolor{cyan!16} \color{blue}yes&\cellcolor{cyan!16} \color{blue} no  \cellcolor{cyan!16} \color{blue}& \cellcolor{cyan!16} \color{blue}yes & \cellcolor{cyan!16} \color{blue}yes, no &\cellcolor{cyan!16} \color{blue} 1 & \cellcolor{cyan!16} \color{blue}single & \cellcolor{cyan!16} \color{blue}yes \\ %\\
				
				\bottomrule 
		\end{threeparttable}
	\end{center}
\end{table*}

\begin{Comment}
\begin{table*}[!h]
	\caption[ \color{blue}Theoritical comparisions with prior-art]{ Scope of the proposed method compared to the state-of-the-art dilution algorithms}
	\label{table:obj_comapare}
	\scriptsize
	%\def\arraystretch{1}
	\begin{center}
		\begin{threeparttable} 
			%\resizebox{\columnwidth}{!}{%
			\begin{tabular}{|p{2.3cm}|p{1.2cm}|p{.85cm}|p{.8cm}|p{.9cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.4cm}|}%p{1cm}|p{1cm}|}%llllllll} 
				\toprule 
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Method}} &
				%			    \parbox[t]{1mm}{\rotatebox[origin=c]{90}{Valve use in mixing channel?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Valve use in mixing channel?}}&
				%			    {\raggedleft \rotatebox{90}{Valve use in mixing channel?}} &
				%                {\raggedleft \rotatebox{90}{Use of valve: on-line / off-line / free?}} & 
				%                \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Use of valve: on-line / off-line / free?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Valve handling mechanism}}&
				%                Valve handling mechanism
				%			    {\raggedleft  \rotatebox{90}{Error scale?}}&
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Error scale?}}&Error-tolerance limit
				%			    
				\cellcolor{pink!16}
				\color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Error-tolerance limit}}&
				%			    {\raggedleft  \rotatebox{90}{Is accuracy similar to accuracy of DMFB?}}&
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is accuracy similar to accuracy of DMFB?}}& 
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering achieves higher accuracy}}&
				%			    {\raggedleft  \rotatebox{90}{Is fluid-injection sequence specific?}} &
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is fluid-injection sequence specific?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Is fluid-injection sequence target-specific?\todo[inline]{I dont understand its meaning}}}&
				%			    {\raggedleft  \rotatebox{90}{Are unused fluid recycled?}}&
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Are unused fluid recycled?\todo[inline]{not important}}}&
				%			    {\raggedleft  \rotatebox{90}{Mix, Split?}} &
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Mix, Split?}}&
				%			    {\raggedleft  \rotatebox{90}{\# used fluid-injection velosity?}} &
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \# used fluid-injection velosity?}}&
				%			    {\raggedleft \rotatebox{90}{\emph{CF}-value at outlet (single / multiple / in a range)?}} &
				%			    \cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \emph{CF}-value at outlet (single / multiple / in a range)?}}&
				%			    # of CF-values produced?
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering \# \emph{CF}-values produced}}&
				%				{\raggedleft \rotatebox{90}{Programmable?}}
				\cellcolor{pink!16} \color{blue}\rotatebox[origin=c]{90}{\parbox[c]{2cm}{\centering Programmable?}}\\ 
				\midrule
				{ \raggedleft Wang {\em et al.}\cite{Philip2016}} & yes (?) & off-line & $>$1\% &no& no &no & yes, yes &  1 & multiple (3) & yes (fixed ratio) \\ 
				
				{ \raggedleft Jeon {\em et al.}\cite{Xmas}} & no & valve-free & undefined &no& ? &no  & yes, yes & 1 & in a range & no \\ \\
				
				{ \raggedleft Lee {\em et al.} \cite{SerialDilution}} & no & free & undefined &no& ?  &no & yes, yes & 1 & multiple (fixed) & no \\ \\ 
				
				{ \raggedleft Bhattacharjee {\em et al.}\cite{Rotary}} & yes & on-line &   &no& ? &no  & yes, yes & 1 & yes & yes \\ \\%(upto certain label) \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{Banerjee2017}} & no & valve-free &  $\leq$ 0.5&yes& yes  &no & yes, no & 2 & single & yes\\ \\% &yes & yes  &no   & yes, no & 2 & single & yes \\ \\
				
				{ \raggedleft Banerjee {\em et al.} \cite{BanerjeeVLSID2019}} & no & valve-free &  $\leq$ 0.5\% &yes& yes  &no & yes, no & 2 & single & yes \\ \\
				
				\cellcolor{cyan!16} \color{blue}{ \raggedleft [Proposed]} & \cellcolor{cyan!16} \color{blue}no & \cellcolor{cyan!16} \color{blue}off-line & \cellcolor{cyan!16} \color{blue} $<$0.5\% &\cellcolor{cyan!16} \color{blue}yes&\cellcolor{cyan!16} \color{blue} no  \cellcolor{cyan!16} \color{blue}& \cellcolor{cyan!16} \color{blue}yes & \cellcolor{cyan!16} \color{blue}yes, no &\cellcolor{cyan!16} \color{blue} 1 & \cellcolor{cyan!16} \color{blue}single & \cellcolor{cyan!16} \color{blue}yes \\ \\
				
				\bottomrule 
			\end{tabular} %}
			%			%\tiny
			%			\begin{tablenotes}
			%				\item[1] all operations within the error-recovery subgraph are assumed to be error-free; $^2$ All split operations will be allowed to perform a fixed number of times and the last one is assumed to be error-free; 
			%				$^3$ Will produce all the target-{\em CF}s at the same time in parallel.
			%			\end{tablenotes}
		\end{threeparttable}
	\end{center}
\end{table*}
\end{Comment}

==> tables/SimulationFramework.tex <==
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{table}[!h]%t]
	\tiny 
	\caption{Computation Platform} 
	\label{tb1:computation_platform}
	\begin{center}
		\begin{tabular}{||>{\small}p{2cm}| >{\small}p{5.2cm}||} 
			\hline
			&\\% &\\
			CPU & Intel Core $i7-3770 $CPU @ $3.40$ GHz,\\& $4$ cores \\%&\\ %[1ex] 
			\hline 
			%&\\ &\\
			Operating System & Windows 10  \\%&\\  %[1ex]
			\hline
			%&\\ &\\
			Software & COMSOL Multiphysics 5.2  \\%[1ex]
			\hline
			%&\\ &\\
			Model Dimension & 3D \\&\\ %[1ex]
			\hline
			% &\\ &\\
			\begin{tabular}{l}
				Materials \\(incompresible\\ Newtonian\\ Fluid) 
			\end{tabular} 
			& Water used as buffer\\%[0.1ex] 
			& \begin{tabular}{|l l|}
				\hline 
				Sample & Diffusion co-efficient of \\& sample in water $[m^2/sec]$ \\ %[1ex]
				\hline
				Ethanol & $1.24\times10^{-9}$\\
				Glycerol & $0.94\times10^{-9}$\\
				\hline
				%Pentane-n & $0.000807$
			\end{tabular} \\%[1ex]
			%&\\ 
			% &\\ &\\
			\hline
			%&\\ &\\
			Used Physics & Laminar flow (SPF: Single Phase Flow) \\ 
			& Transport of diluted species (TDS)\\%&\\ %[1ex]
			\hline
			% &\\ &\\
			Meshing & Predefined element size at\\& extra fine while calibrating fluid dynamics \\ %&\\ % [1ex] 
			\hline
			%&\\ &\\
			Study & Time dependent \\&(Time range: 0 sec - 200 sec\\ &; time step 1 sec) \\%&\\ %[1ex]  
			\hline
			Solver & Direct PARDISCO solver\\%&\\ 
			\hline 
		\end{tabular}
	\end{center}
\end{table}

==> tables/TheoryVSSimulationError.tex <==
 \setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{table*}[!h]%t]
	%\caption{\color{red}{Comparison between Theoretical Errors and Simulation Errors (updated)}} 
	\caption{Comparison between Theoretical Errors and Simulation Errors} 
	\label{tb3:error_compare}
	\begin{center}
		%\begin{tabular}{||c|c|c|c|c||} 
		\begin{tabular}{||>{\small}p{1cm}>{\small}p{2.3cm}|>{\small}p{2.3cm}|>{\small}p{2cm}|>{\small}p{1.8cm}|>{\small}p{2cm}|>{\small}p{1.8cm}|>{\small}p{1.8cm}||} 
			
			\hline \multicolumn{2}{||c|}{}&&&&&&\\
			%\hline [1ex]
			\multicolumn{2}{||c|}{Target CF} & Nearest & Theoretical & Nearest & Theoretical & Simulated & Simulation\\
			\multicolumn{2}{||c|}{\emph{(tCF)}} & tCF& Error for BS & Target CF& Error for FSD &Result&Error\\
			\hhline{--~~~~~~}
			& & for denom $2^6$ & %[\emph{tCF' $ - $ tCF}]
			& \emph{tCF'}&  %[\emph{tCF' $ - $ tCF}] 
			& \emph{tCF''} & %[\emph{tCF'' $ - $ tCF'}]
			\\%&&&&&&&\\
			(in \%) & (in fraction form) &(in fraction form)& (in \%) & (in \%)& (in \%) & (in \%)& (in \%)\\[1ex]
			%A & B & C & D & E & F & G\\
			(A)&(B)&(C)&(C-A)&(D)&(D-A)&(E)&(E-A)%$\frac{\|D-A \| }{A}*100$ \%)
			\\
			%A & B & C & D & E & F & G\\
			\hline
			%\hline
			%&&&&&&&\\
			3 & $\frac{1.92}{64}$ &$\frac{2}{64}$  & +$\frac{0.08}{64}$(=0.13\%)	&	3.13	&	+0.13&	3.125	&	-0.125	\\ %&&&&&&&\\%\hline
			3.25&$\frac{2.08}{64}$&$\frac{2}{64}$&-$\frac{0.08}{64}$(=-0.13\%)	 &	3.23	&	-0.02 &	3.22	&	-0.03	\\ %&&&&&&&\\%\hline
			12.5&$\frac{8}{64}$&$\frac{8}{64}$ &0	&	12.5	&	0 &	12.43	&	-0.07	\\ %&&&&&&&\\%\hline
			31&$\frac{19.84}{64}$&$\frac{20}{64}$ &+$\frac{0.16}{64}$(=0.25\%)	&	31.03	&	+0.03 &	30.75	&	-0.25	\\ %&&&&&&&\\%\hline
			41.75& $\frac{26.72}{64}$&$\frac{27}{64}$&+$\frac{0.28}{64}$(=0.44\%)	 &	41.67	&	-0.08 &	41.598	&	-0.152	\\ %&&&&&&&\\%\hline
			%50.75(=$\frac{32.48}{64}$)&$\frac{32}{64}$ &	50.82	&	+0.07 &-$\frac{0.48}{64}$(=0.75\%)	&	51.8	&	0.98	\\ &&&&&&\\%\hline
			%51(=$\frac{32.64}{64}$)&$\frac{33}{64}$ &	51.02	&	+0.02 &+$\frac{0.36}{64}$(=0.56\%)	&	51.83	&	0.81	\\ &&&&&&\\%\hline
			54.5&$\frac{34.88}{64}$&$\frac{35}{64}$	&+$\frac{0.12}{64}$(=0.19\%)	&54.55	&	+0.05 &	54.63	&	+0.13	\\ %&&&&&&&\\%\hline
			69.3&$\frac{44.375}{64}$&$\frac{44}{64}$ &-$\frac{0.3}{64}$(=-0.47\%)	&	69.23	&	-0.067 &	69.36	&	+0.06	\\ %&&&&&&&\\%\hline
			70&$\frac{44.8}{64}$&$\frac{45}{64}$ &+$\frac{0.2}{64}$(=0.31\%)	&	70	&	0 &	70.2	&	+0.2	\\ %&&&&&&&\\%\hline
			87.5&$\frac{56}{64}$&$\frac{56}{64}$  &0	&	87.5	&	0&	87.52	&	+0.02	\\ %&&&&&&&\\%\hline
			95&$\frac{60.8}{64}$&$\frac{61}{64}$ &+$\frac{0.2}{64}$(=0.31\%)	&	95	&	0 &	95.08	&	+0.08 	\\ \hline
		\end{tabular}
	\end{center}
\end{table*}
